A Sharpness Based Loss Function for Removing Out-of-Focus Blur

The success of modern Deep Neural Network (DNN) approaches can be attributed to the use of complex optimization criteria beyond standard losses such as mean absolute error (MAE) or mean squared error (MSE). In this work, we propose a novel method of utilising a no-reference sharpness metric Q introduced by Zhu and Milanfar for removing out-of-focus blur from images. We also introduce a novel dataset of real-world out-of-focus images for assessing restoration models. Our fine-tuned method produces images with a 7.5 % increase in perceptual quality (LPIPS) as compared to a standard model trained only on MAE. Furthermore, we observe a 6.7 % increase in Q (reflecting sharper restorations) and 7.25 % increase in PSNR over most state-of-the-art (SOTA) methods.

==> removals.tex <==
\begin{figure}%[hbtp]
    %%%% Original Images %%%%
    \begin{subfigure}{0.480\linewidth}
      \includegraphics[width=\linewidth]{MMSP_Example/notice4_cropped.png}
      \caption{Original Image}
      \label{fig:original_image}
    \end{subfigure}\hfill
    %%%% Low Blur Image %%%%
    \begin{subfigure}{0.480\linewidth} 
      \includegraphics[width=\linewidth]{MMSP_Example/notice4_lbc_cropped.png}
      \caption{Low Blur Image}
      \label{fig:lowBlur_image}
    \end{subfigure}
    
    \medskip
    %%%% Med Blur Image %%%%%%%
    \begin{subfigure}{0.480\linewidth}
      \includegraphics[width=\linewidth]{MMSP_Example/notice4_mbc_cropped.png}
      \caption{Medium Blur Image}
      \label{fig:medBlur_image}
    \end{subfigure}\hfill
    %%%% High Blur Image %%%%%
    \begin{subfigure}{0.480\linewidth}
      \includegraphics[width=\linewidth]{MMSP_Example/notice4_hbc_cropped.png}
      \caption{High Blur Image}
      \label{fig:highBlur_image}
    \end{subfigure}

    \caption{Crop from image \texttt{Poster4} from the SigMedia dataset. Top Row: Original Image (Left), Low Blur Image (Right). Bottom Row: Medium Blur Image (Left), High Blur Image (Right).}
    \label{fig:sigmedia_dataset}
\end{figure}


%%%%%%%%% ARCHITECTURE %%%%%%%%%%%%
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Model_Arch/UNet_MMSP.png}
    \caption{Architecture}
    \label{fig:unet_arch}
\end{figure}


As can be seen from table~\ref{tab:comparison_table_artificial}, our method produces sharper images comparable to SOTA and iterative models. Although iterative methods produce images with higher PSNR and perceptual quality, the inference time of such methods is significantly higher. This can be attributed to convergence issues of such methods.
A visual comparison of these methods can be seen in figure AAA. 

